Cactus Representation of Minimum Cuts: Derandomize and Speed up

Given an undirected weighted graph with $n$ vertices and $m$ edges, we give the first deterministic $m^{1+o(1)}$-time algorithm for constructing the cactus representation of \emph{all} global minimum cuts. This improves the current $n^{2+o(1)}$-time state-of-the-art deterministic algorithm, which can be obtained by combining ideas implicitly from three papers [Karger JACM'2000, Li STOC'2021, and Gabow TALG'2016] The known explicitly stated deterministic algorithm has a runtime of $\tilde{O}(mn)$ [Fleischer 1999, Nagamochi and Nakao 2000]. Using our technique, we can even speed up the fastest randomized algorithm of [Karger and Panigrahi, SODA'2009] whose running time is at least $\Omega(m\log^4 n)$ to $O(m\log^3 n)$.

==> 3-main-old.tex <==

\subsubsection{Main algorithm for computing lower vertices}

\label{sec:compute lower main}

-- Valid lower vertex respecting $u$ ==> lower vertices below $u$, $L_u$ 

-- Given a set $S \subseteq V(T)$, highest vertices of $S$ is ....

-- highest vertices of $L_u \setminus \upath{u_1}{u_2}$

In this subsection we state the main algorithm for \Cref{lem:computing-lower-vertex}. %
Recall that the goal is, for every right edge $e$ in $T$, we want to compute its lower vertex $l_e$.


Consider a right edge $e=(u_1, u_2)$ in $T$.
The corresponding minimal 2-respecting mincut $u_e^\downarrow\setminus l_e^\downarrow$ separates both $u_1$ and $u_2$ from the root $r$.
It is not hard to see that the upper vertex $u_e$ has to be an ancestor of $\LCA(u_1, u_2)$ and that the lower vertex $l_e$ should never be on the path between $u_1$ and $u_2$ on $T$.
For convenience, we denote $\upath{v}{w}$ as the set of vertices on the path between any two vertices $v$ and $w$ on $T$.
That is, we have that $l_e$ should never be on $\upath{u_1}{u_2}$.

Recall that for each vertex $v$ we have obtained its highest partner $H(v)$.
Imagine that there is a data structure such that, given a vertex $u$,
the data structure efficiently tells you the set of \emph{maximal} vertices\footnote{This is a very vague intuition: we repeatedly get rid of lower vertex if we find two vertices are comparable to each other. See \Cref{def:maximal-valid-lower-vertex} for a formal definition.} $v$ such that $u\in \upath{v}{H(v)}$. (We say that $u$ is maximal with respect to a set if there is no other $u'$ in the set that is an ancestor of $u$.)
These vertices are called \emph{valid lower vertices respect to $u$} (see \Cref{def:valid-lower-vertex}).
How could we use this data structure for finding a lower vertex $l_e$ for an edge $e$?
Observe that $H(l_e)$ is an ancestor of $u_e$.
If we now stand at the vertex $u_e$ (which we do not know yet) and query the data structure, $l_e$ must appear in the returned set.
However, there are two challenges:
first, the returned set may be large, so searching (and verifying) the actual $l_e$ may be inefficient.
Second,
we do not know exactly which vertex is $u_e$.

Surprisingly, a crucial observation (formally stated in \Cref{lem:uniqueness-of-lower-vertex}) says that,
$l_e$ will be the unique element (after excluding vertices on $\upath{u_1}{u_2}$) returned from the data structure when queried at $u_e$.
This uniqueness property resolves the first challenge.
\Cref{lem:uniqueness-of-lower-vertex} states an even stronger result --- if we query the data structure at any vertex between $\LCA(u_1, u_2)$ and $u_e$ of a right edge $e$, either we find nothing or $l_e$ is uniquely returned!
This observation enables us to resolve the second challenge: 
in order to search for a lower vertex,
the algorithm conceptually climbs up the tree from $\LCA(u_1, u_2)$ and
iteratively checks if the current vertex lies on this 
\emph{canonical path} $\hatP_e := \upath{u_e}{l_e}$.
Maybe one would ask questions such as: ``Why don't we use binary search?'' Unfortunately this seems to be improbable --- our algorithm does not know either $u_e$ or $H(l_e)$ at this moment.






Now, we formally introduce the critical observation, and then we describe the implementation of the algorithm. 
Let us start with defining vertices of our interest when querying at a vertex $u$.

\begin{definition}[Valid Lower Vertex]\label{def:valid-lower-vertex}
    We call a vertex $v$ a \emph{valid lower vertex} respect to $u$ if $v\in u^\Downarrow$ and $\Maximal(v)\in u^\uparrow$.
    In other words, there exists a comparable 2-respecting mincut containing $u$ with the lower vertex $v$. 
\end{definition}

Notice that a valid lower vertex $v$ respect to $u$ may not be the actual lower vertex for a particular right edge $e$. This is simply because that 
(1) $v$ is on the path $\upath{u_1}{u_2}$, or (2) there exists a higher $v'\in v^\uparrow$ that is also a valid lower vertex respect to $u$ so there must be a mincut of smaller size by the crossing property.

As we mentioned before, if we simply ignore all valid lower vertices described above,
in the case that $e$ is the right edge, what remains must be a unique lower vertex and it must be $l_e$. We now formalize the above intuition via \emph{maximal valid lower vertex} and present the most crucial structural property.

\begin{definition}[Maximal Valid Lower Vertex]
\label{def:maximal-valid-lower-vertex}
We say that $v$ is a \emph{maximal valid lower vertex} respect to $u$ in a set $S\subseteq u^{\downarrow}$, if there is no $v'\in S\cap v^\uparrow$ so that $v'$ is also a valid lower vertex.
\end{definition}

\begin{lemma}[Unique Valid Lower Vertex on the Right Tree]
    \label{lem:uniqueness-of-lower-vertex}
    Suppose $e=(u_1, u_2)$ is a right edge. That is, the minimal mincut of $e$ is a comparable 2-respecting mincut $u_e^\downarrow\setminus l_e^\downarrow$. 
    Then, for all $u$ on the path between $u_e$ and $\LCA(u_1, u_2)$, 
    there is at most one maximal valid lower vertex respect to $u$ in $u^\Downarrow\setminus \upath{u_1}{u_2}$. 
    If there exists one maximal valid lower vertex repect to $u$, it must be $l_e$.
\end{lemma}

Therefore, the lower vertex $l_e$ should be highest valid lower vertex $v$ respect to $u$ satisfying $v\in u^\Downarrow\setminus (\upath{u_1}{u_2})$.
The proof of \Cref{lem:uniqueness-of-lower-vertex} is deferred to \Cref{sec:omit}.

\begin{proof}
TODO
\end{proof}

\paragraph{Implementation.}
There are two challenges for us to implement an efficient algorithm that finds all lower vertex of right edges using \Cref{lem:uniqueness-of-lower-vertex}.
The first challenge is to maintain the set of all maximal valid lower vertices respect to a vertex dynamically. The second challenge is that the algorithm does not have enough time to perform queries to maximal valid lower vertices on all ancestors per edge.
The proposed algorithm solves the two challenges above using a one-time post-order traversal, with a little help from the top-tree data structures.



In order to describe our algorithm and address how do we cope with both challenges, we first describe an algorithm that solves a simpler case when there is no need for the algorithm to perform multiple queries to maximal valid lower vertices on the ancestors of $\LCA$ per edge.
After we describe the algorithm that solves the simpler case, we generalize the algorithm and solve both challenges in the general case.


\subsubsection*{Simple Case: $\LCA(u_1, u_2)$ is always on the path $\hatP_{e}$.} 

Suppose that every edge $e=(u_1, u_2)$ is a right edge for tree $T$, and that $\LCA(u_1, u_2)\in \hatP_e$.


While running the post-order traversal, we use a top-tree to maintain all the valid lower vertices respect to the current vertex $u$. And then, we  find the lower vertex $l_e$ for every edge $e = (u_1,u_2)$ with $\LCA(u_1, u_2) = u$ via queries to the top-tree data structure.

The vertex set of the top-tree is the same with the original graph. We shall maintain a value on each vertex with the following invariant. Suppose the current vertex is $u$. For each vertex $v\in u^\downarrow$, if $v$ is a valid lower vertex respect to $u$, the value of $v$ in the top-tree should be $depth_v$ (the depth of $v$ in $T$).
Otherwise, if $v$ is not a valid lower vertex, the value of $v$ is $\infty$.

The algorithm will maintain the invariant above while running the post-order traversal. Initially, the top-tree is the same as the spanning tree with a super large value $\infty \gg n$ assigned on each vertex. When the traversal reach $u$, the algorithm will do the following updates on the top-tree. First, we check for each child $v$ of $u$: if $H(v)\neq \NULL$, then assign value $depth_v$ on vertex $v$, otherwise leave the value of $v$ unchanged (which is $\infty$). Second, for any vertex $v\in u^\downarrow$ such that $H(v)$ is a child of $u$, $v$ will no longer be a valid lower vertex with respect to $u$ and any vertex later in the post-order traversal. Therefore, we assign $\infty$ on the value of these vertices. Since for each vertex $v$ the value of $v$ is changed at most twice in the algorithm, the top-tree can be maintained in $O(n\log n)$ total time.


We show how to use the top-tree to find $l_e$ for each edge $e = (u_1,u_2), \LCA(u_1,u_2)=u$. Recall that the lower vertex $l_e$ is highest valid lower vertex $v$ respect to $u$ satisfying $v\in u^\Downarrow\setminus (\upath{u_1}{u_2})$. We first apply $\cut(u,parent_u)$ to separate the subtree rooted at $u$. And then the lower vertex can be found by $l_e = \MinNonPath(u_1,u_2)$. Finally, we apply $\link(u,parent_u)$ to restore the tree.


\subsubsection*{General Case: $\LCA(u_1, u_2)$ may not be on the path $\hatP_{e}$.}

In the general case, we no longer have the assumption $\LCA(u_1,u_2)\in\hatP_e$. 
Recall that we have stated in the beginning of \Cref{sec:compute lower main} for any edge $e = (u_1,u_2)$ the algorithm climbs up the tree from $\LCA(u_1,u_2)$ and iteratively checks if the current vertex lies on the canonical path $\hatP_e$. But the time cost of performing such multiple queries per edge is unacceptable.

We shall deal with the challenge with the following idea. Again the algorithm runs a one-time post-order traversal. Suppose the current vertex is $u$. For all the edges with both endpoints in $u^\downarrow$ and $u$ is below the path $\hatP_e$\thatchaphol{Define below the path}, the lower vertices of these edges\thatchaphol{what exactly is this set of edges?} have not been found yet. The algorithm will pack these edges together and represent the package using one pointer and forward it to the parent of $u$, since the following key observation guarantees that the minimal mincut of these edges (assuming to be right edges) are the same.



\begin{lemma}\label{lem:general-case-property}
    Fix vertex $u$. For all right edges $e_1, e_2$ where their endpoints are in $u^\downarrow$ and $u\in \hatP_{e_1}^\Downarrow\cap \hatP_{e_2}^\Downarrow$, i.e. $l_{e_1},l_{e_2}\not\in u^\downarrow$, we have that  $\hatP_{e_1}=\hatP_{e_2}$. %
    \thatchaphol{Must use all the predicate in the statement explicitly in the proof.}
\end{lemma}

\begin{proof}
    Suppose for contradiction that $\hatP_{e_1}\neq \hatP_{e_2}$. If the minimal mincut of $e_1$ and the minimal mincut of $e_2$ form a nested structure, WLOG, let $\hatP_{e_1}\subset \hatP_{e_2}$. Then the minimal mincut of $e_1$ will also be a mincut containing $e_2$, which has smaller size than the mincut corresponds to $\hatP_{e_2}$, contradiction. In the other case, $\hatP_{e_1}$ crosses with $\hatP_{e_2}$, then the intersection of these two minimal mincuts will also form a mincut containing them with smaller size, contradiction.
\end{proof}



When the traversal reaches vertex $u$, the algorithm receives a package from each child of $u$.
For each package, the algorithm selects an arbitrary edge $e$ from the package and tests whether $l_e\in u^\downarrow$ using top-tree in the same way as the algorithm that solves the simple case.
By \Cref{lem:general-case-property}, if $l_e\in u^\downarrow$, then all the lower vertices of the edges in the package are $l_e$. Otherwise, none of lower vertices of the edges in the package is in the subtree of $u$, then the edges will be further packed and forwarded to the parent of $u$. The algorithm can pack the edges efficiently using linked list.


We prove that the entire algorithm can be implemented using $O(n+m)$ top-tree queries. For each edge, the algorithm checks whether $l_e\in \LCA(u_1,u_2)$ as stated in the simple case, which takes $O(m)$ queries. And for the general case, in each vertex $u$, the algorithm will make one top-tree query for the package from each child of $u$, which takes $O(n)$ queries for the whole traversal process. Therefore, the algorithm for computing $l_e$ for every edge $e$ can be done in $O(m\log n)$ total time, which proves \Cref{lem:computing-lower-vertex}.

\thatchaphol{Include the proof of Lemma 5.9.}












==> D-applications.tex <==
\section{Applications}\label{app:applications}

\paragraph{Incremental Exact Mincut Problem}

Given an initial graph $G$, the goal of the incremental exact mincut algorithm is to build a data structure that supports edge insertions and queries of mincut value. As mentioned earlier in the introduction,  Our Monte-Carlo cactus construction algorithm in \Cref{thm:main} implies the following result.

\begin{theorem}
\end{theorem}


==> incomparable.tex <==
\section{Minimal incomparable 2-respecting min-cuts of edges}



First, we define the minimal 2-respecting incomparable mincut of vertex or edge.

\begin{definition}
    The minimal 2-respecting incomparable mincut of vertex $u$ is the 2-respecting incomparable mincut $v^\downarrow\cup w^\downarrow$ containing $u$ with the smallest size. If no 2-respecting incomparable mincut seperates $u$ from $r$, then its minimal incomparable mincut is undefined. In the same way, we define the minimal incomparable 2-respecting mincut of edge $e$.
\end{definition}

It turns out that the minimal 2-respecting incomparable mincut of vertices can be found fast enough already.

\begin{lemma}[\cite{karger2009near}]
    Given a tree, labeling all the vertices with the minimal 2-respecting incomparable mincut can be done in $O(m\log^2 n)$ deterministically.
\end{lemma}

Computing the minimal incomparable min-cuts of edges is the main contribution of this section.

\begin{lemma}
    Given a spanning tree $T$, we can  deterministically compute, for each edge $e$, a label representing minimal incomparable min-cuts of $e$ in total time $O(m\log^2 n)$.
\end{lemma}


There are two cases of the minimal incomparable 2-respecting mincut $v^\downarrow\cup w^\downarrow$ of an edge $e = (u_1, u_2)$. First, both $u_1$ and $u_2$ are in the subtree of the same vertex in the 2-respecting cut. WLOG, suppose $u_1, u_2\in v^\downarrow$. We have the following lemma.

\begin{lemma}
    For the minimal incomparable 2-respecting mincut $v^\downarrow\cup w^\downarrow$ of an edge $e = (u_1, u_2)$, if both $u_1, u_2\in v^\downarrow$, then $v^\downarrow\cup w^\downarrow$ is also the minimal incomparable 2-respecting mincut of $\texttt{lca}(u_1, u_2)$.
\end{lemma}

Therefore, we first label edge $e=(u_1,u_2)$ with the minimal incomparable 2-respecting mincut of $\texttt{lca}(u_1, u_2)$. Then we go to the other case to check whether there exists a incomparable 2-respecting mincut of $e$ with smaller size.

In the remaining part of this section, we consider the second case. For edge $e = (u_1, u_2)$ and its minimal incomparable 2-respecting mincut $v^\downarrow\cup w^\downarrow$, we have $u_1\in v^\downarrow$ and $u_2\in w^\downarrow$.

\begin{definition}
    Two cuts $X$ and $Y$ are said to be crossing if each of $X\cap Y, X\setminus Y, Y\setminus X, X^C\cap Y^C$ is non-empty.
\end{definition}

The following crossing property will be used many times throughout the paper.

\begin{lemma} [\cite{dinits1976structure}]
    \label{lem:crossing-mincuts}
    If $X$ and $Y$ are crossing min-cuts, then $X\cap Y, X\setminus Y, Y\setminus X, X\cup Y$ are min-cuts. Further,
    \[
        C(X\cap Y, X^C\cap Y^C) = C(X\setminus Y, Y\setminus X) = 0 ~.
    \]
\end{lemma}

In order to find the minimal 2-respecting mincut of edge, we define the notion of minimal minprecut.

\begin{definition}
    Consider any vertex $\hat v$ on a bough and let $w$ be the minimum precut of $v = \ell(\hat v)$ and let $u$ be a vertex such that $u\in w^\downarrow$. If there doesn't exist $x\in w^\downarrow\cap u^\uparrow$ such that $x$ is also a minimum precut of $v$, then $w$ is said to be a minimal minprecut of $v$ respect to $u$. Moreover, suppose $e=(v',u)$ where $v'$ is a descendant of $v$ on the bough, then $w$ is said to be a minimal minprecut of $v$ respect to $e$ if it is minimal minprecut of $v$ respect to $u$.
\end{definition}
\hezt{picture.}

Interestingly, we find that the maximal minprecut is also useful in our algorithm. We define it in a similar way. In our algorithm, the minimal minprecut is always found by the oracle $\texttt{MinPath}$ while the maximal minprecut is always found by $\texttt{MinPath}^-$, since there is a difference on the $val[w]$ with a positive and negative $\epsilon$ multiplied by the depth of $w$.
\begin{definition}
    Consider any vertex $\hat v$ on a bough and let $w$ be the minimum precut of $v = \ell(\hat v)$ and let $u$ be a vertex such that $u\in w^\downarrow$. If there doesn't exist $x\in w^\uparrow$ such that $x$ is also a minimum precut of $v$, then $w$ is said to be a maximal minprecut of $v$ respect to $u$. Moreover, suppose $e=(v',u)$ where $v'$ is a descendant of $v$ on the bough, then $w$ is said to be a maximal minprecut of $v$ respect to $e$ if it is maximal minprecut of $v$ respect to $u$.
\end{definition}

We first exploit the structure of minimal min-cut of edges for the incomparable case.
\begin{lemma}
    \label{lem:incomparable-minimal-2-respect-mincut-monotone}
    Suppose the minimal min-cut of edge $e=(u_1,u_2)$ 2-respects a tree $T$, where it is represented by vertices $v$ and $w$, $v\perp w$, $u_1\in v^\downarrow$ and $u_2\in w^\downarrow$. Then $w$ is the minimal minprecut of $v$ respect to $e$. Furthermore, there doesn't exist $v'\in u_1^\uparrow\cap v^\Downarrow$ and $w'\in u_2^\uparrow$, such that $v'$ and $w'$ forms another 2-respecting incomparable min-cut separating $e$ from $r$.
\end{lemma}

\begin{proof}
    First, $w$ is the minimal minprecut of $v$ respect to $e$, else there is a smaller min-cut separating $e$ from root $r$. Next, if there exists $v'\in u_1^\uparrow\cap v^\downarrow \setminus\{v\}, w'\in u_2^\uparrow$ and $v'\perp w'$, such that $v'^\downarrow\cup w'^\downarrow$ forms another 2-respecting min-cut separating $e$ from $r$, then the intersection of $v^\downarrow\cup w^\downarrow$ and $v'^\downarrow\cup w'^\downarrow$ is a smaller min-cut that separating $e$ from $r$, contradiction.
\end{proof}



Following Lemma~\ref{lem:incomparable-minimal-2-respect-mincut-monotone}, we are able to state the process of labeling the minimal min-cut of edges. Suppose edge $e = (u_1,u_2)$
, we will find the deepest $v\in u_1^\uparrow$ such that $C(v^\downarrow) + C_{v}$ is the value of min-cut and there exists a minimal minprecut $w$ of $v$ respect to $e$. Then $v^\downarrow\cup w^\downarrow$ is the minimal incomparable min-cut of $e$ that cutting an edge on the bough.

This leads to the recursive structure of our algorithm. We process the vertices on the bough from the leaf to the top (In Algorithm~\ref{alg:label-incomparable}  line~\ref{code:label-incomparable-recursive}). After returning from the child of $v$, we call the \texttt{LocalUpdate} (Algorithm~\ref{alg:local-update}) on the current vertex $v$. \texttt{LocalUpdate} will update $val[w]$ (and also $val^+[w], val^-[w]$) by calling \texttt{AddPath} on the endpoints of edges from $v$. $val[w]$ will be the precut $C_v(w)$ when \texttt{LocalUpdate} is completed.

We use a binary-search-tree to store the edges that have not found their minimal incomparable mincut yet. Note that there's only one global binary-search-tree in \Cref{alg:label-incomparable}.

\begin{itemize}
    \item \texttt{InsertBST}$(x, e)$, store edge $e$ into the BST using index $x$, where $x$ is the pre-order of some vertex $u$.
    \item \texttt{ExtractBst}$(w^{\downarrow})$, extract all the edges with index in the subtree of $w$.
\end{itemize}

Consider the current vertex $\hat v$ on the bough and the leader $v = \ell(\hat v)$. If the value $C(v^\downarrow) + C_v$ equals to the minimum cut, then we shall enumerate the minprecut $w$ of $v$ and label all the edges below $w$ and $v$ by extracting the edges in the \texttt{BST} using $\texttt{ExtractBST}(w^\downarrow)$. This procedure is done by \Cref{alg:mincut-subtree-update}.

Note that above is only the sketch of the algorithm and the time cost has not been taken in consideration. Below, we shall define outer vertex which will be crucial for both the correctness and time analysis of our algorithm.

\begin{definition}
    For each contracted vertex $\hat v$ on a bough, let $\hat u$ be the top vertex of this bough. Define $t(\hat v)$ to be the leader of the top vertex on the bough, i.e. $t(\hat v) := \ell(\hat u)$.
\end{definition}

\begin{definition}
    We call $w$ an outer vertex of $\hat{v}$ if $w\not\in t(\hat v)^\downarrow$.
\end{definition}

\thatchaphol{Need picture.}

The outer minprecut is defined similar as minprecut except that only the outer vertices are taken in consideration.

\begin{definition}
    \label{def:outer-minprecut}
    The outer minprecut of $\hat v$ is defined as the minimum precut $w$ of $v$ such that $w$ is an outer vertex of $v$, denoted as $C'_v$. Specifically,
    \[
        C'_v = \min\{C_v(w)\mid w\not\in t(l^{-1}(v))^\downarrow,  \exists(v',w')\in E, v'\in v^\downarrow, w'\in w^\downarrow\}
    \]
\end{definition}

In our algorithm, we shall consider outer minprecut instead of minprecut. It turns out that outer minprecut is sufficient for identifying the minimal incomparable mincut for edges, since the following lemma holds.

\begin{lemma}
    \label{lem:incomparable-outer-guarantee}
    For any pair of incomparable vertices $v$ and $w$, either $v$ is an outer vertex of $w$ or $w$ is an outer vertex of $v$. %
\end{lemma}


This lemma is a basic property of heavy-light decomposition that can be easily checked by drawing figures of the incomparable vertices $v$ and $w$ and their corresponding contracted vertex and bough. We defer the proof to Appendix~\Cref{app:?}.


Before presenting our algorithm, we show some key invariants that we shall maintain throughout our algorithm. Suppose we are processing vertex $\hat v$ on the bough, let $v = \ell^{-1}(v)$, we have

\begin{enumerate}[label=Invariant \arabic*., leftmargin=*]
    \item $val[w]= C_v(w)$ for every outer vertex $w$ of $v$.
    \item $val^* = C'_v$.
    \item The set $P$ contains all the maximal outer minprecuts of $v$ that respect some edge $e\in \texttt{BST}$.
\end{enumerate}


\begin{algorithm}[H]
    \caption{\texttt{LocalUpdate$(\hat v)$}}
    \label{alg:local-update}
    \begin{algorithmic}[1]
        \State Call \texttt{AddPath}$(\ell(\hat v),\infty)$.
        \label{code:set-ancestor-infinity}
        \For{each edge $e=(\hat v,u)$ such that $u\not\in t(\hat v)^\downarrow$}
            \State Call \texttt{InsertBST}$(pre\_order[u], e)$.
            \State Call \texttt{AddPath}$(u,-2C(\hat v,u))$.
            \label{code:add-path}
            \State Call $w\gets \texttt{MinPath}(u)$.
            \State $val^* \gets \min\{val^*, val[w]\}$.
            \label{code:outer-minprecut-value-update}
        \EndFor
        \State If $val^*$ is changed in the previous line, set $P = \emptyset$.
        \label{code:local-update-P-reset}
        \State Set $P \gets P \cup \{ w \mid val[w] = val^*, \exists (\hat v,u)\in E, w = \texttt{MinPath}^-(u) \}$.
        \label{code:P-update}
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
    \caption{\texttt{MinCutUpdate$(w', \hat v)$}}
    \label{alg:mincut-subtree-update}
    \begin{algorithmic}[1]
        \While{$e = (v',u)\gets \texttt{ExtractBst}(w'^{\downarrow})$}
            \State $w\gets \texttt{MinPath}(u)$.
            \State Update the label of minimal 2-respecting mincut of edge $e$ if the size of $\ell(\hat v)^\downarrow\cup w^\downarrow$ is smaller than the mincut containing $e$ that found before.
        \EndWhile
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
    \caption{\texttt{LabelIncomparable$(\hat v)$}}
    \label{alg:label-incomparable}
    \begin{algorithmic}[1]
        \State Call \texttt{LabelIncomparable}$(\hat u)$ recursively on $\hat v$'s child $\hat u$ in the bough.
        \label{code:label-incomparable-recursive}
        \State Call \texttt{LocalUpdate}$(\hat v)$. \label{code:label-incomparable-local-update}
        \If{$C(\ell(\hat v)^{\downarrow}) + val^* = MinCut$}
        \label{code:label-incomparable-mincut-check}
            \State For each $w\in P$, call \texttt{MinCutUpdate}$(w, \hat v)$.
            \label{code:label-incomparable-extract-PS}
            \State Set $P = \emptyset$.
            \label{code:label-incomparable-P-reset}
        \EndIf
    \end{algorithmic}
\end{algorithm}

We defer the proof of these invariants to \Cref{sec:invariants}. We first prove that Invariants 2 and 3 implies the correctness of the algorithm.

\begin{lemma}%
    \label{lem:incomparable-correct-label}
    Suppose the minimal min-cut of edge $e = (u_1,u_2)$ 2-respects a tree T, where it is represented by incomparable vertices $v$ and $w$. WLOG by \Cref{lem:incomparable-outer-guarantee}, we suppose $w$ is an outer vertex of $v$. After running Algorithm~\ref{alg:label-incomparable} on the top vertex of the bough containing $\hat v = \ell^{-1}(v)$, the label of edge $e$ will be the minimal incomparable  min-cut $v^\downarrow\cup w^\downarrow$ of $e$.
\end{lemma}

\begin{proof}
    Consider the stage that $v$ is on the bough. By Invariants 2 and 3, in \Cref{alg:label-incomparable}, when returning from $\texttt{LocalUpdate}(\hat v)$, it guarantees that $val^* = C'_v$ and $P$ contains the maximal minprecuts of $v$ respect to all the edge $e\in \texttt{BST}$.
    
    First, we show that $e\in \texttt{BST}$. First, $e$ is inserted to the BST when \Cref{alg:label-incomparable} reaching vertex $l^{-1}(u_1)$. Then prove by contradiction, suppose $e$ is popped out before reaching $\hat v$. Then there exists $v'\in v^\Downarrow$ and $w'$, such that $v'^\downarrow\cup w'^\downarrow$ is also a mincut containing $e$. But this contradicts to \Cref{lem:incomparable-minimal-2-respect-mincut-monotone}. Therefore, $e\in \texttt{BST}$ when returning from $\texttt{LocalUpdate}(\hat v)$.
    
    Then in line~\ref{code:label-incomparable-mincut-check}, the value $C(v^\downarrow) + val^*$ equals to the mincut by the assumption of the lemma. In the next step, there exists a vertex $w'$ is extracted such that $w'\in w^\uparrow$ since $w'$ is a maximal minprecut respect to $e$. And the \texttt{MinCuttreeUpdate}$(w',\hat v)$ is called. Therefore, $e$ is extracted in \Cref{alg:mincut-subtree-update} and labeled by $v^\downarrow\cup w^\downarrow$.
\end{proof}

\subsection{Invariants}
\label{sec:invariants}

We prove Invariants 1-3 in this subsection. First, \Cref{lem:outer-precut-value} shows the correctness of Invariants 1 and 2.

\begin{lemma}
    \label{lem:outer-precut-value}
    In \Cref{alg:label-incomparable}, When returning from \texttt{LocalUpdate}$(\hat v)$, let $v = \ell(\hat v)$, we have
    \begin{enumerate}
        \item $val[w]=C_v(w)$ for every outer vertex $w$ of $v$.
        \item $val^* = C'_v$.
    \end{enumerate}
\end{lemma}


The lemma is an analogue of Lemma~7.9 in \cite{karger2000minimum}. The proof is almost verbatim same with the proof in Karger's paper. For completeness, we include the proof here.

\begin{proof}
    Prove by induction. First, we consider the base case that $\hat v$ is the leaf of a bough. In line~\ref{code:set-ancestor-infinity}, we assign an infinity $val[w]$ to every ancestor $w$ of $v$, as required in the definition of $C_v(w)$. Next, $2C(v,u)$ is substracted in line~\ref{code:add-path} from every $val[w]$ such that $u\in w^\downarrow$ for $u\not\in t(v)$. Therefore, the total amount substracted from $val[w]$ is $2C(v,w^\downarrow)$, as required in \Cref{def:precut}. In the end, $val[w] = C_v(w)$ for every $w\not\in t(v)^\downarrow$. For Claim 2, in line~\ref{code:outer-minprecut-value-update}, $val^*$ minimizes over $w\perp v$ that are ancestors of neighbors of $v$, this will identify $C_v$ according to \Cref{def:outer-minprecut}.
    
    Now suppose $v$ has a child $u$. After calling \texttt{LabelIncomparable}$(u)$, we know by induction that $val[w] = C_u(w)$. Thus, after executing \texttt{LocalUpdate}$(v)$, which decreases each $val[w]$ by $2C(v,w^\downarrow)$ for $w\not\in t(v)^\downarrow$, entry $val[w]$ is updated to be
    \begin{align*}
        C_u(w) - 2C(v,w^\downarrow)
        &
        = (C(w^\downarrow) - 2C(u^\downarrow,w^\downarrow)) - 2C(v,w^\downarrow) \\
        &
        = C(w^\downarrow) - 2C(v\cup u^\downarrow, w^\downarrow) \\
        &
        = C(w^\downarrow) - 2C(v^\downarrow, w^\downarrow) \\
        &
        = C_v(w)
    \end{align*}
    Next, we prove Claim 2. Suppose $v$ has a child $u$. According to \Cref{lem:outer-minprecut-inherited}, there are two possibilities for $C'_v$. One possibility is that $C'_v = C'_u$. By induction, the recursive call to \texttt{LabelIncomparable}$(u)$ sets $val^* = C'_u$. On the other hand, if $C'_v\neq C'_u$, then by \Cref{lem:outer-minprecut-inherited}, $C'_v = C_v(w)$ for an ancestor of an outer neighbour of $v$. Then $val^*$ is set to $C'_v$ by $\texttt{LocalUpdate}(v)$.
\end{proof}

In the rest of this subsection, we aim for proving Invariant 3. First, we show a key property of outer minprecut.

\begin{lemma}
    \label{lem:outer-minprecut-inherited}
    Let $v$ be a vertex in $T$ and $\hat v = \ell^{-1}(v)$. Suppose $w$ is an outer minprecut of $v$. If $\hat v$ is a leaf in $T'$, then there exists an edge between $\hat v$ and $w^\downarrow$. On the other hand, if $\hat v$ is a non-leaf in $T'$, let $\hat u$ be the only child of $\hat v$ in $T'$ and $u = \ell(\hat u)$. Then either there exists an edge between $\hat v$ and $w^\downarrow$, or $w$ is an outer minprecut of $u$.
\end{lemma}

\begin{proof}
    If $\hat v$ is a leaf in $T'$, then by definition of a minprecut of $v$, $\hat v$ and $w^\downarrow$ must be connected. Otherwise, suppose there is no edge between $\hat v$ and $w^\downarrow$, then we need to prove that $w$ is an outer minprecut of $u$. By contradiction, suppose $w$ is not an outer minprecut of $u$, then $\exists w'\not\in t(\hat u)^\downarrow$, $C_u(w') < C_u(w)$. By definition
    $t(\hat u) = t(\hat v)$, we also have $\exists w'\not\in t(\hat v)^\downarrow$. Since there is no edge between $\hat v$ and $w^\downarrow$, $C_v(w) = C_u(w)$. Then we get $C_v(w') \le C_u(w') < C_u(w) = C_v(w)$, which means that $w$ cannot be an outer minprecut of $v$, contradiction.
\end{proof}

\begin{remark}
    Note that the condition that $w$ is an \emph{outer} minprecut of $v$ in \Cref{lem:outer-minprecut-inherited} is necessary in the proof. If $w'\in t(\hat v)^\downarrow$, then there is a case that $w'\in v^\downarrow\setminus u^\downarrow$. Then $w'$ is a $u$-preuct but not a $v$-precut, and the contradiction is invalid.
\end{remark}

Finally, we prove Invariant 3 for the set $P$.

\begin{lemma}
    In \Cref{alg:label-incomparable}, when returning from $\texttt{LocalUpdate}(\hat v)$, the set $P$ contains all the maximal minprecuts of $v$ respect to any the edge $e\in \texttt{BST}$.
\end{lemma}

\begin{proof}
    By induction, we assume that when returning from the recursive call in \Cref{alg:label-incomparable}, the set $P$ contains the maximal minprecuts of $v$ respect to all the edge $e\in \texttt{BST}$. Note that this assumption vacuously holds for the base case since \texttt{BST} is empty.
    
    What we need prove are two folds. First, we prove that when returning from $\texttt{LocalUpdate}(\hat v)$, $P$ contains all the maximal minprecuts of $v$ respect to any edge $e\in \texttt{BST}$. Second, we prove that this condition also holds when \Cref{alg:label-incomparable} finishing processing $v$, to meet the induction hypothesis.
    
    To prove the first claim, we separate it into two cases depend on $val^*$ whether changed in $\texttt{LocalUpdate}(\hat v)$. Suppose $val^*$ changed, then for any the outer minprecut $w$ of $v$, there exists an edge between $\hat v$ and $w^\downarrow$ by \Cref{lem:outer-minprecut-inherited}. Therefore, all the maximal minprecuts are identified in Line~\ref{code:P-update}. For the second case that $val^*$ remains the same, then $P$ is unioned with all the maximal minprecuts of the edges which are neighbours of $v$. For each edge $e\in \texttt{BST}$ that is not the neighbour of $v$, the maximal minprecut of $e$ is already in $P$ by induction hypothesis and \Cref{lem:outer-minprecut-inherited}. Therefore, the condition holds for both cases.
    
    Next, we prove the condition also holds when \Cref{alg:label-incomparable} finishing processing $v$. If the check of mincut failed in line~\ref{code:label-incomparable-mincut-check}, then $P$ remains the same and nothing need to prove. Suppose the check of mincut passes, then the only modification of $P$ is in line~\ref{code:label-incomparable-P-reset}. By the first claim, when returning from $\texttt{LocalUpdate}(\hat v)$, $P$ contains all the maximal minprecuts of $v$ respect to any edge $e\in \texttt{BST}$. Since for each maximal minprecut $w$ of $v$, all the edges with an endpoint in $w^\downarrow$ are extracted in $\texttt{MinCutUpdate}(w,\hat v)$, there is no minprecuts of $v$ respect to any edge in \texttt{BST} any more. Hence let $P = \emptyset$ satisfies the condition.
\end{proof}



\subsection{Time complexity of labeling minimal incomparable 2-respecting min-cuts of edges}

We show that the objective of Section~\ref{sec:label-incomparable} can be achieved in $O(m\log^2 n)$ by our algorithm.

\begin{lemma}
    The minimal incomparable min-cut that 2-respects a tree can be labeled in $O(m\log^2 n)$ time for all the edges.
\end{lemma}

Recall that we achieve this by running $O(\log n)$ iterations and in each iteration, we invoke Algorithm~\ref{alg:label-incomparable} at the topmost vertex of each bough. Define degree of a bough $d(B)$ to be the number of edges incident to the bough. We show that the time of Algorithm~\ref{alg:label-incomparable} working on a bough $B$ is $O(d(B)\log n)$. Since each edge is connected to at most two bough, the total time cost of one iteration can be bounded by $O(m\log n)$. Therefore, the time of the overall $O(\log n)$ iterations for a tree is bounded by $O(m\log^2 n)$.

Now we focus on a bough $B$ to show the amortized time of Algorithm~\ref{alg:label-incomparable} on $B$ is $O(d(B)\log n)$. Algorithm~\ref{alg:label-incomparable} starts with calling \texttt{LocalUpdate} on current vertex $v$. In \texttt{LocalUpdate}, the operations \texttt{AddPath} and \texttt{MinPath} are implemented by dynamic tree and the updates cost of $val^*$ and $P$ is linear to the degree of vertex $v$. Therefore the cost of \texttt{LocalUpdate} on vertex $v$ is $O(d(v)\log n)$. Then we come to the part where we actually label the minimal incomparable 2-respecting min-cuts for edges.

For the for loop processing $P$ in line~\ref{code:label-incomparable-extract-PS} of \Cref{alg:label-incomparable}, the cost is amortized by the number of edges incident to the bough since there is at most one minprecut inserted to $P$ for each edge. In \Cref{alg:mincut-subtree-update}, the amortized cost is $O(d(B)\log n)$. Combining together, the time cost of processing a bough is $O(d(B)\log n)$.

Therefore, the overall time complexity is $O(m\log^2 n)$.



==> mincut-algo.tex <==
\section{Modified mincut algorithm}

\label{sec:modified-mincut-algorithm}

In this section, We review Karger's min-cut algorithm from \cite{karger2000minimum} and then extend it for our purpose. Suppose we have a set of tree packing such that every min-cut 2-respects some tree in the tree packing. The problem now becomes given a spanning tree $T$, finding the min-cuts that 2-respects $T$. 

\subsection{Incomparable 2-respecting mincut}

\begin{definition}
    $C(X,Y)$ is the sum of weights of edges with one end-point in vertex set $X$ and the other in vertex set $Y$. (An edge with both endpoints in $X\cap Y$ is counted twice.) Overloading our notation, $C(S) = C(S,V-S)$.
\end{definition} 

For any pair of incomparable vertices $w\perp v$,
\[
    C(v^\downarrow\cup w^\downarrow) = C(v^\downarrow) + C(w^\downarrow) - 2C(v^\downarrow,w^\downarrow) ~.
\]

\begin{definition}
    \label{def:precut}
    The $v$-precut at $w$, denoted by $C_v(w)$, is the value
    \[
        C_v(w) = C(v^\downarrow\cup w^\downarrow) - C(v^\downarrow) = C(w^\downarrow) - 2C(v^\downarrow,w^\downarrow)
    \]
    if $w\perp v$ and $\infty$ otherwise.
\end{definition}

\begin{definition}
    The minimum $v$-precut, denoted $C_v$, is the value 
    \[
        \min\{ C_v(w)\mid \exists(v',w')\in E, v'\in v^\downarrow, w'\in w^\downarrow \} ~.
    \]
\end{definition}

\begin{lemma}[\cite{karger2000minimum}]
    If it is determined by incomparable vertices, the minimum cut is $\min_v(C(v^\downarrow)+C_v)$.
\end{lemma}

For completeness, we copy Karger's proof here.

\begin{proof}
    Let the minimum cut be induced by $v$ and a vertex $w\perp v$. It suffices to show that $w$ is in the set over which we minimize to define $C_v$ in \Cref{def:precut}. But this follows from the fact that each side of the minimum cut induces a connected subgraph of $G$, for this implies that there must be an edge $(v', w')$ from $v^\downarrow$ to $w^\downarrow$. To see that each side of the minimum cut must be connected, note that if one side of the minimum cut has two disconnected components then we can reduce the cut value by moving one of these components to the other side of the cut.
\end{proof}

Karger further restricts the problem locally on a bough, which is an approach similar with heavy-light decomposition.

\begin{definition}
    A bough is a maximal path on a tree that contains a leaf at one end and all the other vertices have degree 2 in the tree.
\end{definition}

After contracting all the boughs into the parent of its top vertex, the total number of leaves is at most a half of that in the original tree. Hence, in $O(\log n)$ iterations, the tree will be contracted into a single vertex. The problem is now restricted to find the strictly 2-respecting min-cuts where one of the edges is on a bough.

\thatchaphol{It is not clear why it should be here.}
\zhongtian{I move it here. Previously it is in the beginning of the section.}

Since $C(v^\downarrow)$ can be calculating in linear time, the rest is only $C_v$ for each vertex. We achieve this by maintaining a value $val[w]$ at each vertex $w$. While we scan vertex $v$ on the bough from bottom to top, the value $val[w]$ will always be updated to the precut $C_v(w)$. $val[w]$ can be maintained by dynamic tree in near-linear time \cite{sleator1983data}.

We simultaneously maintain the value $val^+[w]$ and $val^-[w]$  such that $val^+[w] = val[w] + \epsilon|w^\downarrow|$ and $val^-[w] = val[w] - \epsilon|w^\downarrow|$, where $\epsilon$ is some constant smaller than $1/n$. This can be done by running $\texttt{AddPath}(v,\epsilon)$ for each vertex as a pre-processing step, where $\texttt{AddPath}(v,x)$ is an operation that adding $x$ to $val[u]$ for each $u\in v^\uparrow$. And $\texttt{MinPath}(v)$ refers to find the minimum $val^+$ from $v$ to the root. We maintain the following operations using dynamic tree.


\begin{itemize}
    \item $\texttt{AddPath}(v,x)$: add $x$ to $val[u]$ (also $val^+[u]$ and $val^-[u]$) for every $u\in v^\uparrow$.
    \item $\texttt{MinPath}(v)$: return $\arg\min_{u\in v^\uparrow} val^+[u]$.
    \item $\texttt{MinPath}^-(v)$: return $\arg\min_{u\in v^\uparrow} val^-[u]$.
\end{itemize}

Karger's original algorithm has $O(\log n)$ iterations where the tree $T$ is contracted progressively. Suppose the minimal min-cut of an edge $e=(u_1,u_2)$ is defined by $v$ and $w$, where $v\perp w$, $u_1\in v^\downarrow$ and $u_2\in w^\downarrow$, then our goal is to identify this min-cut in the phase that $v$ is on a bough. 

Since $w^\downarrow$ may not correspond to a subtree in the contracted tree, we need to maintain two trees. One is the contracted tree $T'$. The other is the original tree $T$ where we maintain $val$ and find the minprecuts.

\begin{definition}
    Each vertex $\hat v$ in the contracted tree $T'$ represents a set of vertices in the original tree $T$. For each such vertex $\hat v$, let $\ell(\hat v)$ denote the leader of the set, which is the vertex of least depth in $T$. Conversely, each vertex $v$ in the original tree $T$ is the leader of a contracted vertex on a bough in $T'$ in some phase, denote this set by $\ell^{-1}(v)$.
\end{definition}

In the whole paper, we follow the convention that $\hat u$ and $\hat v$ represent the vertices on the contracted tree $T'$, while $u,v$ and $w$ represent the vertices on the original tree $T$.



\subsection{Comparable 2-respecting mincut}


For any pair of comparable vertices $v\in w^\downarrow$,
\[
    C(w^\downarrow - v^\downarrow) = C(w^\downarrow) - C(v^\downarrow) + 2(C(v^\downarrow,w^\downarrow) - C(v^\downarrow,v^\downarrow)) ~.
\]

Suppose vertex $v$ is on the bough, we consider each $w\in v^\uparrow$. Let $val[w] = C(w^{\downarrow}) + 2C(v^\downarrow,w^\downarrow)$. Again we use dynamic tree to maintain $val[w]$ and find the minimal $val[w]$. Similar with the previous section, we maintain $val^+[w] = val[w] + \epsilon|w^\downarrow|$ and $val^-[w] = val[w] - \epsilon|w^\downarrow|$.

Here comes the difference with the incomparable case. We only need one \texttt{MinPath} query after the local update on the current vertex $v$ to find the minimum $val[w]$ above $v$. In this way, we can find the comparable 2-respecting min-cuts.

Next, we do some preparation for our main algorithm. For each vertex $v$, we use $\texttt{MinPath}^-(v)$ to find the highest $w$ such that $w^\downarrow\setminus v^\downarrow$ forms a min-cut. The highest such $w$ for each $v$ is denoted by $H(v)$.


==> old-section-6.1.tex <==

\subsection{Minimum $v$-Precuts and $P$-Outer Minimum $v$-Precuts}
\label{sec:min-v-precut-and-p-outer-min-v-precut}
\thatchaphol{My impression: a lot of definitions but the reader will have no idea why he need to read it. We need some explanation why we define these things}

Fix a spanning tree $T\in {\cal T}$. 
Our algorithm for \Cref{lem:label-incomparable-path} requires implementation on efficiently identifying incomparable 2-respecting mincuts $v^\downarrow\cup w^\downarrow$ with one vertex $v$ on the path $P\in\cP$.
In this section we first recall the concepts of \emph{minprecut values} from~\cite{karger2000minimum} and then we 
introduce \emph{outer minprecut values} that help us to describe the algorithm with clarity.

Observe that for any pair of incomparable vertices $v\perp w$, the weight of the cut induced by $v^\downarrow\cup w^\downarrow$ can be expressed as
\[
    \C(v^\downarrow\cup w^\downarrow) = \C(v^\downarrow) + \C(w^\downarrow) - 2\C(v^\downarrow,w^\downarrow) ~.
\]

Suppose $v^\downarrow$ is one part\shangen{not precise.} of the minimal 2-respecting mincut of $e$.
Then by factoring out the terms only related to $v$, it suffices to compute the following \emph{incomparable precut values} for all $v\perp w$.

\begin{definition}[Incomparable precut value]
    The \emph{incomparable precut value} of $v$ at $w$, is defined by 
    \[
        \CI_v(w) := \C(w^\downarrow) - 2\C(v^\downarrow,w^\downarrow) ~.
    \]
    Note that the value is only defined in the incomparable scenario $v\perp w$.
\end{definition}


The incomparable precut values are defined analogously to the comparable precut values. Actually, they share the same functionality in the sense that given a vertex $v$, an algorithm can be designed to find a \emph{partner} $w$ such that $v$ and $w$ together idetifies a incomparable (resp. comparable) 2-respecting mincut $v^\downarrow\cup w^\downarrow$ (resp. $w^\downarrow\setminus v^\downarrow$).



Consider a path $P$ in a path decomposition $\cP$, our algorithm designed for \Cref{lem:label-incomparable-path} will ``climb up'' $P$ from the deepest vertex to the highest vertex. Meanwhile, it maintains the precut value of $v$ at all the incomparable vertices $w\perp v$ and the minprecut value of $v$ stated below, so that the algorithm can find the partners of $v$ efficiently.

\begin{definition}
    The \emph{incomparable minprecut value} of $v$, is defined by
    \[
        \CI_v := \min\{ \CI_v(w)\mid \exists(v',w')\in E, v'\in v^\downarrow, w'\in w^\downarrow \} ~.
    \]
\end{definition}

Here, it requires a technical constraint that
there is at least one edge between $v^\downarrow$ and $w^\downarrow$.
The most important reason is that when we process a path $P$ we can only afford a cost related to $|E(P^\downarrow)|$.

The algorithm is then able to update the minprecut values by scanning 


First, for the running time analysis, the algorithm needs to charge on the edges when it computes the minprecut. %

Second for the correctness, only certain vertices of $w$ are candidates for forming incomparable 2-respecting mincut with $v$, as stated in the following lemma.

\begin{lemma}[\cite{karger2000minimum}]
    If there exists some mincut that is a incomparable 2-respecting cut, then the weight of the mincut is $\min_v(\C(v^\downarrow)+\CI_v)$.
\end{lemma}





A vertex $w$ is called an \emph{incomparable mincut partner} of $v$ if $v^\downarrow\cup w^\downarrow$ is a mincut. For brevity, we will omit the word ``comparable/incomparable'' and simply call $\CI_v(w)$ as precut value of $v$ (at $w$) and call $w$ a \emph{mincut partner} of $v$ if the context is clear. Besides, we call $w$ a \emph{minprecut partner} of $v$ if $\CI_v(w) = \CI_v$. Note that a mincut partner must be a minprecut partner, but it may not be correct conversely.

Given a path $P\in \cP$, our algorithm should maintain the minprecut value of the current vertex $v$ when climbing up the path $P$. It turns out that if we further exclude all the candidates of partner within $P^\downarrow$, the algorithm can maintain minprecut values and partners of $v$ in a more efficient way, which leads to the following definitions.

\begin{definition}
    We call $w$ an outer vertex of path $P$ if $w\not\in P^\downarrow$.
\end{definition}

The \emph{outer minprecut value} is defined similar to the minprecut value except that only the outer vertices are taken in consideration.

\begin{definition}
    \label{def:outer-minprecut}
    The \emph{$P$-outer minprecut value} of $v$ is defined as the minprecut value of $v$ such that the minprecut partner $w$ is an outer vertex of $v$. Specifically,
    \[
        \CI_{v,P} = \min\{\CI_v(w)\mid w\notin P^\downarrow,  \exists(v',w')\in E, v'\in v^\downarrow, w'\in w^\downarrow\}
    \]
\end{definition}

We call $w$ a \emph{$P$-outer minprecut partner} of $v$ if $w$ is an outer vertex of $P$ and $\CI_{v,P}(w) = \CI_{v,P}$.
Now we are ready to describe the algorithm.

